A Formalization and Proof of the Extended Church-Turing Thesis -Extended Abstract-

We prove the Extended Church-Turing Thesis: Every effective algorithm can be efficiently simulated by a Turing machine. This is accomplished by emulating an effective algorithm via an abstract state machine, and simulating such an abstract state machine by a random access machine, representing data as a minimal term graph.

==> eptcsdata.tex <==
\providecommand{\firstpage}{72}
\providecommand{\publicationstatus}{E. Kashefi, J. Krivine, F. van Raamsdonk (Eds.) \\
DCM 2011\\
EPTCS 88, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.88.6}{10.4204/EPTCS.88.6}}

